OlmoEarth: Stable Latent Image Modeling for Multimodal Earth Observation

Earth observation data presents a unique challenge: it is spatial like images, sequential like video or text, and highly multimodal. We present OlmoEarth: a multimodal, spatio-temporal foundation model that employs a novel self-supervised learning formulation, masking strategy, and loss all designed for the Earth observation domain. OlmoEarth achieves state-of-the-art performance compared to 12 other foundation models across a variety of research benchmarks and real-world tasks from external partners. When evaluating embeddings OlmoEarth achieves the best performance on 15 out of 24 tasks, and with full fine-tuning it is the best on 19 of 29 tasks. We deploy OlmoEarth as the backbone of an end-to-end platform for data collection, labeling, training, and inference of Earth observation models. The OlmoEarth Platform puts frontier foundation models and powerful data management tools into the hands of non-profits and NGOs working to solve the world's biggest problems. OlmoEarth source code, training data, and pre-trained weights are available at $\href{https://github.com/allenai/olmoearth_pretrain}{\text{https://github.com/allenai/olmoearth_pretrain}}$.

==> ai2style/defns.tex <==
%
% A useful set of commands
\usepackage{mathtools}
\usepackage{dsfont}
\usepackage[dvipsnames]{xcolor}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage{booktabs}
\usepackage{xfrac}
\usepackage{bbm}

\usepackage{algpseudocode}
\usepackage{algorithm}
\usepackage{algorithmicx}

\usepackage[most]{tcolorbox}
\usepackage{xparse}
\usepackage{lipsum}
\usepackage{changepage}
\usepackage{enumitem}

\newcommand{\qedwhite}{\hfill \ensuremath{\Box}}

%http://www-db.stanford.edu/~manku/latex.html
%The itemize environment can be replaced by:
\newcommand{\squishlist}{
   \begin{list}{$\bullet$}
    { \setlength{\itemsep}{0pt}      \setlength{\parsep}{3pt}
      \setlength{\topsep}{3pt}       \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{1.5em} \setlength{\labelwidth}{1em}
      \setlength{\labelsep}{0.5em} } }

\newcommand{\squishlisttwo}{
   \begin{list}{$\bullet$}
    { \setlength{\itemsep}{0pt}    \setlength{\parsep}{0pt}
      \setlength{\topsep}{0pt}     \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{2em} \setlength{\labelwidth}{1.5em}
      \setlength{\labelsep}{0.5em} } }

\newcommand{\squishend}{
    \end{list}  }

%Example usage: \squishlist    %% \begin{itemize}
%\item First item
%\item Second item
%\squishend     %% \end{itemize}

\newcommand{\denselist}{\itemsep 0pt\topsep-6pt\partopsep-6pt}


\newtheorem{thm}{Theorem}[section]
\newtheorem{cor}{Corollary}[section]
\newtheorem{defn}{Definition}[section]
\newenvironment{mythm}{{\bf Theorem}}{}



\newcommand{\tm}{\tilde{m}}
\newcommand{\tv}{\tilde{v}}

% For bold vector symbols
\newcommand{\myvec}[1]{\boldsymbol{#1}}
\newcommand{\myvecsym}[1]{\boldsymbol{#1}}
\newcommand{\ind}[1]{\mathbb{I}(#1)}

\newcommand{\vzero}{\myvecsym{0}}
\newcommand{\vone}{\myvecsym{1}}
\newcommand{\valpha}{\myvecsym{\alpha}}
\newcommand{\vbeta}{\myvecsym{\beta}}
\newcommand{\vchi}{\myvecsym{\chi}}
\newcommand{\vdelta}{\myvecsym{\delta}}
\newcommand{\vDelta}{\myvecsym{\Delta}}
\newcommand{\vepsilon}{\myvecsym{\epsilon}}
\newcommand{\vell}{\myvecsym{\ell}}
\newcommand{\veta}{\myvecsym{\eta}}
\newcommand{\vgamma}{\myvecsym{\gamma}}
\newcommand{\vGamma}{\myvecsym{\Gamma}}
\newcommand{\vmu}{\myvecsym{\mu}}
\newcommand{\vnu}{\myvecsym{\nu}}
\newcommand{\vkappa}{\myvecsym{\kappa}}
\newcommand{\vlambda}{\myvecsym{\lambda}}
\newcommand{\vLambda}{\myvecsym{\Lambda}}
\newcommand{\vLambdaBar}{\overline{\vLambda}}
\newcommand{\vomega}{\myvecsym{\omega}}
\newcommand{\vOmega}{\myvecsym{\Omega}}
\newcommand{\vphi}{\myvecsym{\phi}}
\newcommand{\vPhi}{\myvecsym{\Phi}}
\newcommand{\vpi}{\myvecsym{\pi}}
\newcommand{\vpsi}{\myvecsym{\psi}}
\newcommand{\vPsi}{\myvecsym{\Psi}}
\newcommand{\vtheta}{\myvecsym{\theta}}
\newcommand{\vTheta}{\myvecsym{\Theta}}
\newcommand{\vsigma}{\myvecsym{\sigma}}
\newcommand{\vSigma}{\myvecsym{\Sigma}}
\newcommand{\vtau}{\myvecsym{\tau}}
\newcommand{\vupsilon}{\myvecsym{\upsilon}}
\newcommand{\vxi}{\myvecsym{\xi}}

\newcommand{\vxn}{\vx^{(n)}}

\newcommand{\vmuY}{\vb}
\newcommand{\vmuMu}{\vmu_{x}}
\newcommand{\vmuMuGivenY}{\vmu_{x|y}}
\newcommand{\vSigmaMu}{\vSigma_{x}}
\newcommand{\vSigmaMuInv}{\vSigma_{x}^{-1}}
\newcommand{\vSigmaMuGivenY}{\vSigma_{x|y}}
\newcommand{\vSigmaMuGivenYinv}{\vSigma_{x|y}^{-1}}
\newcommand{\vSigmaY}{\vSigma_{y}}
\newcommand{\vSigmaYinv}{\vSigma_{y}^{-1}}

%\newcommand{\vmuY}{\vmu_{y}}
%\newcommand{\vmuMu}{\vmu_{\mu}}
%\newcommand{\vmuMuGivenY}{\vmu_{\mu|y}}
%\newcommand{\vSigmaMu}{\vSigma_{\mu}}
%\newcommand{\vSigmaMuInv}{\vSigma_{\mu}^{-1}}
%\newcommand{\vSigmaMuGivenY}{\vSigma_{\mu|y}}
%\newcommand{\vSigmaMuGivenYinv}{\vSigma_{\mu|y}^{-1}}
%\newcommand{\vSigmaY}{\vSigma_{y}}
%\newcommand{\vSigmaYinv}{\vSigma_{y}^{-1}}

\newcommand{\muY}{\mu_{y}}
\newcommand{\muMu}{\mu_{\mu}}
\newcommand{\muMuGivenY}{\mu_{\mu|y}}
\newcommand{\SigmaMu}{\Sigma_{\mu}}
\newcommand{\SigmaMuInv}{\Sigma_{\mu}^{-1}}
\newcommand{\SigmaMuGivenY}{\Sigma_{\mu|y}}
\newcommand{\SigmaMuGivenYinv}{\Sigma_{\mu|y}^{-1}}
\newcommand{\SigmaY}{\Sigma_{y}}
\newcommand{\SigmaYinv}{\Sigma_{y}^{-1}}

\newcommand{\hatf}{\hat{f}}
\newcommand{\haty}{\hat{y}}
\newcommand{\const}{\mbox{const}}
\newcommand{\sigmoid}{\mbox{sigm}}

\newcommand{\one}{(1)}
\newcommand{\two}{(2)}

\newcommand{\va}{\myvec{a}}
\newcommand{\vb}{\myvec{b}}
\newcommand{\vc}{\myvec{c}}
\newcommand{\vd}{\myvec{d}}
\newcommand{\ve}{\myvec{e}}
\newcommand{\vf}{\myvec{f}}
\newcommand{\vg}{\myvec{g}}
\newcommand{\vh}{\myvec{h}}
\newcommand{\vj}{\myvec{j}}
\newcommand{\vk}{\myvec{k}}
\newcommand{\vl}{\myvec{l}}
\newcommand{\vm}{\myvec{m}}
\newcommand{\vn}{\myvec{n}}
\newcommand{\vo}{\myvec{o}}
\newcommand{\vp}{\myvec{p}}
\newcommand{\vq}{\myvec{q}}
\newcommand{\vr}{\myvec{r}}
\newcommand{\vs}{\myvec{s}}
\newcommand{\vt}{\myvec{t}}
\newcommand{\vu}{\myvec{u}}
\newcommand{\vv}{\myvec{v}}
\newcommand{\vw}{\myvec{w}}
\newcommand{\vws}{\vw_s}
\newcommand{\vwh}{\hat{\vw}}
\newcommand{\vx}{\myvec{x}}
%\newcommand{\vx}{\myvec{x}}
\newcommand{\vxt}{\myvec{\tilde{x}}}
\newcommand{\vy}{\myvec{y}}
\newcommand{\vyt}{\myvec{\tilde{y}}}
\newcommand{\vz}{\myvec{z}}

\newcommand{\vA}{\myvec{A}}
\newcommand{\vB}{\myvec{B}}
\newcommand{\vC}{\myvec{C}}
\newcommand{\vD}{\myvec{D}}
\newcommand{\vE}{\myvec{E}}
\newcommand{\vF}{\myvec{F}}
\newcommand{\vG}{\myvec{G}}
\newcommand{\vH}{\myvec{H}}
\newcommand{\vI}{\myvec{I}}
\newcommand{\vJ}{\myvec{J}}
\newcommand{\vK}{\myvec{K}}
\newcommand{\vL}{\myvec{L}}
\newcommand{\vM}{\myvec{M}}
\newcommand{\vN}{\myvec{N}}
\newcommand{\vO}{\myvec{O}}
\newcommand{\vP}{\myvec{P}}
\newcommand{\vQ}{\myvec{Q}}
\newcommand{\vR}{\myvec{R}}
\newcommand{\vS}{\myvec{S}}
\newcommand{\vT}{\myvec{T}}
\newcommand{\vU}{\myvec{U}}
\newcommand{\vV}{\myvec{V}}
\newcommand{\vW}{\myvec{W}}
\newcommand{\vX}{\myvec{X}}
%\newcommand{\vXs}{\vX_{\vs}}
\newcommand{\vXs}{\vX_{s}}
\newcommand{\vXt}{\myvec{\tilde{X}}}
\newcommand{\vY}{\myvec{Y}}
\newcommand{\vZ}{\myvec{Z}}


\newcommand{\vxtest}{\myvec{x}_*}
\newcommand{\vytest}{\myvec{y}_*}


\newcommand{\ftrue}{f_{true}}

\newcommand{\myprec}{\mbox{prec}}
\newcommand{\precw}{\lambda_{w}} % precision of weights (alpha)
\newcommand{\precy}{\lambda_{y}} % precision of y (beta)
\newcommand{\fbar}{\overline{f}}
\newcommand{\xmybar}{\overline{x}}
\newcommand{\ybar}{\overline{y}}
\newcommand{\zbar}{\overline{z}}
\newcommand{\vxbar}{\overline{\vx}}
\newcommand{\vXbar}{\overline{\vX}}
\newcommand{\vybar}{\overline{\vy}}
\newcommand{\vYbar}{\overline{\vY}}
\newcommand{\vzbar}{\overline{\vz}}
\newcommand{\vZbar}{\overline{\vZ}}
\newcommand{\xbar}{\overline{x}}
\newcommand{\Xbar}{\overline{X}}
\newcommand{\Ybar}{\overline{Y}}
\newcommand{\Gbar}{\overline{G}}
\newcommand{\Jbar}{\overline{J}}
\newcommand{\Lbar}{\overline{L}}
\newcommand{\Nbar}{\overline{N}}
%\newcommand{\Qbar}{\overline{Q}}
\newcommand{\Qbar}{\overline{Q}}
\newcommand{\Tbar}{\overline{T}}
\newcommand{\Sbar}{\overline{S}}
\newcommand{\vSbar}{\overline{\vS}}
\newcommand{\Rbar}{\overline{R}}

\newcommand{\vtaubar}{\overline{\vtau}}
\newcommand{\vtbar}{\overline{\vt}}
\newcommand{\vsbar}{\overline{\vs}}

\newcommand{\htilde}{\tilde{h}}
\newcommand{\vhtilde}{\tilde{\vh}}
\newcommand{\Dtilde}{\tilde{D}}
\newcommand{\Ftilde}{\tilde{F}}
\newcommand{\wtilde}{\tilde{w}}
\newcommand{\ptilde}{\tilde{p}}
\newcommand{\pemp}{p_{emp}}
\newcommand{\pstar}{p^*}
\newcommand{\xtilde}{\tilde{x}}
\newcommand{\Xtilde}{\tilde{X}}
\newcommand{\ytilde}{\tilde{y}}
\newcommand{\Ytilde}{\tilde{Y}}
\newcommand{\vxtilde}{\tilde{\vx}}
\newcommand{\vytilde}{\tilde{\vy}}
\newcommand{\ztilde}{\tilde{\z}}
\newcommand{\vztilde}{\tilde{\vz}}
\newcommand{\vthetaMAP}{\hat{\vtheta}_{MAP}}
\newcommand{\vthetaS}{\vtheta^{(s)}}
\newcommand{\vthetahat}{\hat{\vtheta}}
\newcommand{\thetahat}{\hat{\theta}}
\newcommand{\thetabar}{\overline{\theta}}
\newcommand{\vthetabar}{\overline{\vtheta}}
\newcommand{\pibar}{\overline{\pi}}
\newcommand{\vpibar}{\overline{\vpi}}


%\newcommand{\subsubsubsection}[1]{\paragraph{#1}}
\newcommand{\choice}[2]{\left(\!\!\! \begin{array}{c} #1 \\ #2\end{array} \!\!\!\right)}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\defeq}{\stackrel{\rm def}{=}}
\newcommand{\real}{\mathbb{R}}

\newcommand{\given}{\|}
\newcommand{\indep}[2]{{#1} \perp {#2}}
\newcommand{\condindep}[3]{{#1} \perp {#2} | {#3}}
\newcommand{\condindepG}[3]{{#1} \perp_G {#2} | {#3}}
\newcommand{\condindepP}[3]{{#1} \perp_p {#2} | {#3}}
\newcommand{\depend}[2]{{#1} \not \perp {#2}}
\newcommand{\conddepend}[3]{{#1} \not \perp {#2} | {#3}}

\newcommand{\trans}[1]{{#1}^{\mathtt{T}}}
\newcommand{\inv}[1]{{#1}^{-1}}

\newcommand{\ra}{\rightarrow}
\newcommand{\lra}{\leftrightarrow}
\newcommand{\Ra}{\Rightarrow}
%\newcommand{\rv}{r.v.}
\newcommand{\la}{\leftarrow}
\newcommand{\tr}{\mbox{tr}}
\newcommand{\st}{\mbox{  s.t.  }}

\newcommand{\dom}{\mbox{dom}}
\newcommand{\bel}{\mbox{bel}}
\newcommand{\dsep}{\mbox{dsep}}
\newcommand{\sep}{\mbox{sep}}
\newcommand{\entails}{\models}
\newcommand{\range}{\mbox{range}}
\newcommand{\myspan}{\mbox{span}}
\newcommand{\nullspace}{\mbox{nullspace}}
\newcommand{\adj}{\mbox{adj}}

\newcommand{\nbd}{\mbox{nbd}}
\newcommand{\nbr}{\mbox{nbr}}
\newcommand{\anc}{\mbox{anc}}
\newcommand{\desc}{\mbox{desc}}
\newcommand{\pred}{\mbox{pred}}
\newcommand{\nondesc}{\mbox{nondesc}}
\newcommand{\pa}{\pi}
\newcommand{\ch}{\mbox{ch}}
\newcommand{\mb}{\mbox{mb}}
\newcommand{\connects}{\sim}


\newcommand{\betadist}{\mbox{Beta}}
\newcommand{\Betadist}{\mbox{Beta}}
\newcommand{\bernoulli}{\mbox{Ber}}
\newcommand{\Ber}{\mbox{Ber}}
\newcommand{\Binom}{\mbox{Bin}}
\newcommand{\NegBinom}{\mbox{NegBinom}}
\newcommand{\binomdist}{\mbox{Bin}}
\newcommand{\cauchy}{\mbox{Cauchy}}
\newcommand{\DE}{\mbox{DE}}
\newcommand{\Dir}{\mbox{Dir}}
\newcommand{\discrete}{\calM}
\newcommand{\Discrete}{\calM}
\newcommand{\expdist}{\mbox{Exp}}
\newcommand{\expon}{\mbox{Expon}}
\newcommand{\gammadist}{\mbox{Ga}}
\newcommand{\Ga}{\mbox{Ga}}
\newcommand{\gauss}{{\cal N}}
\newcommand{\IG}{\mbox{IG}}
\newcommand{\IGauss}{\mbox{InvGauss}}
\newcommand{\IW}{\mbox{IW}}
\newcommand{\Laplace}{\mbox{Lap}}
\newcommand{\Mu}{\mbox{Mu}}
\newcommand{\Multi}{\mbox{Mu}}
\newcommand{\NIX}{NI\chi^2}
\newcommand{\GIX}{NI\chi^2}
\newcommand{\NIG}{\mbox{NIG}}
\newcommand{\GIG}{\mbox{NIG}}
\newcommand{\NIW}{\mbox{NIW}}
\newcommand{\GIW}{\mbox{NIW}}
\newcommand{\MVNIW}{\mbox{NIW}}
\newcommand{\NW}{\mbox{NWi}}
\newcommand{\MVNIG}{\mbox{NIG}}
\newcommand{\NGdist}{\mbox{NG}}
\newcommand{\prob}{p}
\newcommand{\Poi}{\mbox{Poi}}
\newcommand{\Student}{{\cal T}}
\newcommand{\student}{{\cal T}}
\newcommand{\Wishart}{\mbox{Wi}}
\newcommand{\Wi}{\mbox{Wi}}
\newcommand{\unif}{\mbox{U}}
\newcommand{\etr}{\mbox{etr}}

\newcommand{\softmax}{\calS}
\newcommand{\soft}{\mbox{soft}}
\newcommand{\cond}{\mbox{cond}}
\newcommand{\sign}{\mbox{sign}}
\newcommand{\sgn}{\mbox{sgn}}
\newcommand{\iid}{\mbox{iid}}
\newcommand{\mle}{\mbox{mle}}
\newcommand{\myiff}{\mbox{iff}}
\newcommand{\pd}{\mbox{pd}}
\newcommand{\pdf}{\mbox{pdf }}
\newcommand{\cdf}{\mbox{cdf}}
\newcommand{\pmf}{\mbox{pmf}}
\newcommand{\wrt}{\mbox{wrt}}
\newcommand{\matlab}{{\sc MATLAB}}
\newcommand{\NETLAB}{{\sc NETLAB}}
\newcommand{\MLABA}{\mbox{PMTK}}
\newcommand{\BLT}{\mbox{PMTK}}
\newcommand{\PMTK}{\mbox{PMTK}}
\newcommand{\mywp}{\mbox{wp}}

\newcommand{\KLpq}[2]{\mathrm{KL}\left[{#1}\|{#2}\right]}
\newcommand{\KL}{\mbox{KL}}
\newcommand{\MI}{\mathbb{I}}
\newcommand{\MIxy}[2]{\mathbb{I}\left({#1};{#2}\right)}
\newcommand{\MIxyz}[3]{\mathbb{I}\left({#1};{#2}|{#3}\right)}
\newcommand{\entropy}[1]{\mathbb{H}\left({#1}\right)}
\newcommand{\entropypq}[2]{\mathbb{H}\left({#1}, {#2}\right)}


\newcommand{\vvec}{\mbox{vec}}
\newcommand{\kron}{\otimes}
\newcommand{\dof}{\mbox{dof}}
%\newcommand{\E}{E}
\newcommand{\E}{\mathbb{E}}
\newcommand{\energy}{E}
\newcommand{\expectAngle}[1]{\langle #1 \rangle}
%\newcommand{\expect}[1]{\mathbb{E}\left[ {#1} \right]}
\newcommand{\expect}[2]{\mathds{E}_{{#1}} \left[ {#2} \right]}
\newcommand{\expectGiven}[3]{\mathds{E}_{{#1}} \left[ {#2} \mid {#3} \right]}
\newcommand{\Var}{\mbox{Var}}
\newcommand{\VarGiven}[3]{\mbox{Var}_{{#1}}\left[ {#2} \mid {#3}\right]}
%\newcommand{\Var}{\mathbb{V}}
\newcommand{\var}[1]{\mbox{var}\left[{#1}\right]}
\newcommand{\std}[1]{\mbox{std}\left[{#1}\right]}
\newcommand{\varQ}[2]{\mbox{var}_{{#2}}\left[{#1}\right]}
\newcommand{\cov}[1]{\mbox{cov}\left[{#1}\right]}
%\newcommand{\mode}[1]{\mbox{mode}\left[{#1}\right]}
\newcommand{\median}[1]{\mbox{median}\left[{#1}\right]}



\newcommand{\diag}{\mbox{diag}}
\newcommand{\blkdiag}{\mbox{blkdiag}}
\newcommand{\bias}{\mbox{bias}}
\newcommand{\union}{\cup}
\newcommand{\intersect}{\cap}

\newcommand{\size}{\mbox{size}}
\newcommand{\trace}{\mbox{trace}}


\newcommand{\myc}{c}
\newcommand{\myi}{i}
\newcommand{\myj}{j}
\newcommand{\myk}{k}
\newcommand{\myn}{n}
\newcommand{\myq}{q}
\newcommand{\mys}{s}
\newcommand{\myt}{t}


\newcommand{\supp}{\mbox{supp}}


\newcommand{\calA}{{\cal A}}
\newcommand{\calB}{{\cal B}}
\newcommand{\calC}{{\cal C}}
\newcommand{\calD}{{\cal D}}
\newcommand{\calDx}{{\cal D}_x}
\newcommand{\calE}{{\cal E}}
\newcommand{\cale}{{\cal e}}
\newcommand{\calF}{{\cal F}}
\newcommand{\calG}{{\cal G}}
\newcommand{\calH}{{\cal H}}
\newcommand{\calHX}{{\cal H}_X}
\newcommand{\calHy}{{\cal H}_y}
\newcommand{\calI}{{\cal I}}
\newcommand{\calK}{{\cal K}}
\newcommand{\calM}{{\cal M}}
\newcommand{\calN}{{\cal N}}
\newcommand{\caln}{{\cal n}}
\newcommand{\calNP}{{\cal NP}}
\newcommand{\calMp}{\calM^+}
\newcommand{\calMm}{\calM^-}
\newcommand{\calMo}{\calM^o}
\newcommand{\Ctest}{C_*}
\newcommand{\calL}{{\cal L}}
\newcommand{\calP}{{\cal P}}
\newcommand{\calq}{{\cal q}}
\newcommand{\calQ}{{\cal Q}}
\newcommand{\calR}{{\cal R}}
\newcommand{\calS}{{\cal S}}
\newcommand{\calSstar}{\calS_*}
\newcommand{\calT}{{\cal T}}
\newcommand{\calV}{{\cal V}}
\newcommand{\calv}{{\cal v}}
\newcommand{\calX}{{\cal X}}
\newcommand{\calY}{{\cal Y}}

\newcommand{\Lone}{$\ell_1$}
\newcommand{\Ltwo}{$\ell_2$}

\newcommand{\mya}{\mbox{a}}
\newcommand{\myat}{\alpha_{t|t-1}}
\newcommand{\score}{\mbox{score}}
\newcommand{\AIC}{\mbox{AIC}}
\newcommand{\BIC}{\mbox{BIC}}
\newcommand{\BICcost}{\mbox{BIC-cost}}
\newcommand{\scoreBIC}{\mbox{score-BIC}}
\newcommand{\scoreBICL}{\mbox{score-BIC-L1}}
\newcommand{\scoreL}{\mbox{score-L1}}

\newcommand{\ecoli}{\mbox{{\it E. coli}}}
\newcommand{\doPearl}{\mbox{do}}
\newcommand{\data}{\calD}
\newcommand{\model}{\calM}
\newcommand{\dataTrain}{\calD_{\mbox{train}}}
\newcommand{\dataTest}{\calD_{\mbox{test}}}
\newcommand{\dataValid}{\calD_{\mbox{valid}}}
\newcommand{\futuredata}{\tilde{\calD}}
\newcommand{\algo}{\calA}
\newcommand{\fitAlgo}{\calF}
\newcommand{\predictAlgo}{\calP}
\newcommand{\err}{\mbox{err}}
\newcommand{\logit}{\mbox{logit}}
\newcommand{\parent}{\mbox{pa}}


%%%%%%%%%%% Hoyt

\newcommand{\conv}[1]{\,\,\,\displaystyle{\operatorname*{\longrightarrow}^{\,_{#1}\,}}\,\,\,}
\newcommand{\dconv}{\conv{D}}
\newcommand{\pconv}{\conv{P}}
\newcommand{\asconv}{\conv{AS}}
\newcommand{\lpconv}[1]{\conv{L^{#1}}}

\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{n}


\newcommand{\condSet}{\mathcal{S}}
\newcommand{\condSetC}{\mathcal{\lnot S}}



==> math_commands.tex <==
\newcommand*\diff{\mathrm{d}}
\newcommand*\Image{\mathrm{Im}}
\newcommand*\NN{\smash{\hat{\mathcal{F}}_{\scriptsize\textrm{NN}}}}

\newcommand*\X{\mathcal{X}}
\newcommand*\Z{\mathcal{Z}}
\newcommand*\G{\mathcal{G}}
\newcommand*\D{\mathcal{D}}
\newcommand*\F{\mathcal{F}}
\newcommand*\R{\mathcal{R}}
\newcommand*\TR{\hat{R}}
\newcommand*\Deltab{\bar{\Delta}}
\newcommand*\h{h}
\newcommand*\biasb{\mathrm{bias}}
\newcommand*\varb{\mathrm{var}}
\newcommand*\covb{\mathrm{cov}}
\newcommand*\M{\mathcal{M}}
\newcommand*\B{\mathcal{B}}
\newcommand*\W{\mathcal{W}}
\newcommand*\Loss{\mathcal{L}}
\newcommand*{\Ftr}{\smash{\mathcal{F}_{\scriptsize\textrm{tr}}}}
\newcommand*{\Fts}{\smash{\mathcal{F}_{\scriptsize\textrm{ad}}}}
\newcommand*{\Dtr}{\smash{\mathcal{D}_{\scriptsize\textrm{tr}}}}
\newcommand*{\Dts}{\smash{\mathcal{D}_{\scriptsize\textrm{ad}}}}
\newcommand*{\Etr}{\smash{\mathcal{E}_{\scriptsize\textrm{tr}}}}
\newcommand*{\Ead}{\smash{\mathcal{E}_{\scriptsize\textrm{ad}}}}

\newcommand*{\eg}{e.g.,\@\xspace}
\newcommand*{\versus}{vs.\@\xspace}
\newcommand*{\sut}{s.t.\@\xspace}
\newcommand*{\ie}{i.e.,\@\xspace}
\newcommand*{\iid}{ID\@\xspace}
\newcommand*{\sota}{SoTA\@\xspace}
\newcommand*{\ood}{OOD\@\xspace}
\newcommand*{\metric}{metric}
\newcommand*{\wrt}{w.r.t.\@\xspace}
\newcommand*{\iif}{i.i.f.\@\xspace}
\newcommand*{\aka}{a.k.a.\@\xspace}
\newcommand*{\rhs}{r.h.s.\@\xspace}
\newcommand*{\etc}{etc.\@\xspace}
\newcommand*{\cf}{cf.\@\xspace}
\newcommand*{\resp}{resp.\@\xspace}

\newcommand*\er{\mathrm{er}}
\newcommand*\ess{\operatorname{ess}}

\let\originalleft\left
\let\originalright\right
\renewcommand{\left}{\mathopen{}\mathclose\bgroup\originalleft}
\renewcommand{\right}{\aftergroup\egroup\originalright}

\let\up\textsuperscript
\let\vec\boldsymbol


\newcommand{\defeq}{\mathrel{:\mkern-0.25mu=}}
\newcommand{\eqdef}{\mathrel{=\mkern-0.25mu:}}

\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

\newcommand{\newterm}[1]{{\bf #1}}
\def\figref#1{figure~\ref{#1}}
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\trifigref#1#2#3#4{figures \ref{#1}, \ref{#2}, and \ref{#3}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
\def\secref#1{section~\ref{#1}}
\def\Secref#1{Section~\ref{#1}}
\def\Termref#1{Term~\ref{#1}}
\def\twosecref#1#2{sections \ref{#1} and \ref{#2}}
\def\trisecref#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
\def\appref#1{appendix~\ref{#1}}
\def\Appref#1{Appendix~\ref{#1}}
\def\suppref#1{supp.~\ref{#1}}
\def\Suppref#1{Supp.~\ref{#1}}
\def\eqref#1{eq.~\ref{#1}}
\def\Eqref#1{Eq.~\ref{#1}}
\def\plaineqref#1{\ref{#1}}
\def\chapref#1{chapter~\ref{#1}}
\def\Chapref#1{Chapter~\ref{#1}}
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
\def\algref#1{algorithm~\ref{#1}}
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
\def\partref#1{part~\ref{#1}}
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\Tabref#1{Table~\ref{#1}}
\def\tabref#1{table~\ref{#1}}
\def\twotabref#1#2{tables \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}

\newcommand{\Lp}{\mathcal{L}^\text{prior}}
\newcommand{\Ll}{\mathcal{L}^\text{likeli}}
\newcommand{\Lal}{\Ls^{\text{l}\widehat{\text{ikel}}\text{i}}}

\def\eps{{\varepsilon}}


\def\xopt{{x^{*}}}
\def\Gopt{{G^{*}}}

\def\p{{\textnormal{p}}}
\def\P{{\textnormal{p}}}
\def\Q{{\textnormal{q}}}
\def\q{{\textnormal{q}}}

\def\gTh{{\hat \gT}}
\def\gDh{{\hat \gD}}
\def\gPh{{\hat \gP}}
\newcommand{\tin}[1]{\mbox{\tiny $#1$}}


\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\reps{{\mathcal{E}}}
\def\rtheta{{\Theta}}
\def\rx{{X}}
\def\ry{{Y}}
\def\rz{{Z}}


\def\S{\mathcal{S}}
\def\T{\mathcal{T}}
\def\X{\mathcal{X}}
\def\Y{\mathcal{Y}}
\def\U{\mathcal{U}}

\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}
\def\rvtheta{{\bm{\theta}}}

\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmx{{\mathbf{x}}}
\def\rmy{{\mathbf{y}}}
\def\rmz{{\mathbf{Z}}}

\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}
\def\valpha{{\bm{\alpha}}}
\def\vtheta{{\bm{\theta}}}
\def\vdelta{{\bm{\delta}}}
\def\vDelta{{\bm{\Delta}}}
\def\vmu{{\bm{\mu}}}
\def\vphi{{\bm{\phi}}}
\def\vSigma{{\bm{\Sigma}}}
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\E{{\mathcal{E}}}
\def\mBeta{{\bm{\beta}}}
\def\mTheta{{\bm{\theta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}

\def\tx{{\tens{x}}}


\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gGh{{\hat\gG}}
\def\gFh{{\hat\gF}}


\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathcal{X}}}
\def\sY{{\mathcal{Y}}}
\def\sZ{{\mathcal{Z}}}
\def\sTheta{{\bm{\Theta}}}

\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\pdata}{p_{\rm{data}}}
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}
\newcommand{\dd}{\mathrm{d}}

\newcommand{\laplace}{\mathrm{Laplace}} %

\newcommand{\KL}{$\mathrm{KL}$\@\xspace}
\newcommand{\Kl}{\mathrm{KL}}
\newcommand{\Esp}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\slerp}{\mathrm{slerp}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\Span}{\mathrm{Span}}
\newcommand{\card}{\mathrm{card}}


\newcommand{\KLD}[2]{D_{\mathrm{KL}} \left( \left. \left. #1 \right|\right| #2 \right) }
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}



\newcommand{\parents}{Pa} %

\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}
\newcommand{\acc}{\mathrm{Acc}}
\newcommand{\1}{\mathds{1}}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Earth observation foundation models are advancing quickly~\cite{astruc2024anysat, clayfoundation, wang2025towards, fuller2024croma, siméoni2025dinov3, tseng2025galileo, waldmann_shah_2025_panopticon, tseng2023lightweight, szwarcman2024prithvi, bastani2023satlaspretrain, jakubik2025terramindlargescalegenerativemultimodality, feng2025tessera, brown2025alphaearth}.
Most of these models adopt approaches that have worked for natural image domains.
Earth datasets are aligned, multi-modal, and multi-temporal; naive masking and contrastive setups create overly easy prediction settings with many trivial negatives.
This blunts representation quality.
There is a need for Earth-specific learning objectives and masking strategies.
The limitations of existing modeling challenges are hard to assess since evaluation for such models have remained fragmented: there is no consistently applied test suite.
Reported results often vary in protocol and tuning, making apples-to-apples comparisons difficult.
Even when strong checkpoints exist, adoption, especially outside well-resourced labs, lags due to the end-to-end plumbing required to acquire, harmonize, and fine-tune Earth data at scale.

% several practical issues have prevented their widely-scale adoption. First, training objectives are split into two camps: supervised pretraining on labeled rasters and self-supervised learning on unlabeled imagery. The field lacks a simple, unified recipe that is both stable and high-performing. Pixel-space methods tend to be stable yet semantically limited, while latent-space methods often learn better features but do not generalize to new downstream tasks~\cite{}. 




We present {\model}; a state-of-the-art multi-modal, spatio-temporal Earth observation foundation model.
{\model} addresses these aforementioned issues with a simple, scalable \textbf{self-supervised learning formulation} designed specifically for Earth observation data. 
We also \textbf{comprehensively evaluate} our formulation compared with $12$ baseline model families across $39$ downstream tasks, including research benchmarks and  real-world applications. 
{\model} is \textbf{fully open}: we open source the training code, model weights, and training data. Additionally, we release an end-to-end platform to drive adoption, putting {\model} and powerful
data management tools into the hands of non-profits and NGOs working to solve the world’s biggest problems. 
    

\noindent\textbf{Self-supervised formulation.}
Existing Earth observation foundation models either train to predict supervised labels (like land cover maps from satellite observations~\cite{bastani2023satlaspretrain,mo2024connecting}) or train with unlabeled data in a self-supervised manner~\cite{wang2023ssl4eo,assran2023self,wei2024towards}. 
Our formulation unifies supervised pretraining on labeled rasters and self-supervised learning on unlabeled imagery.
We introduce Latent Masked Image Modeling of Linear Invariant Token Embeddings (\textit{Latent MIM LITE}), which is a simplification of Latent MIM \cite{wei2024towards} that leads to stable training and better performance.
We replace the target encoder of Latent MIM with a linear projection from image patches to token space. 
This simple modification stabilizes training but maintains the representative power of modeling in latent space.



\noindent\textit{Masking Earth observations.}
Many foundation models build upon work in domains like image or text processing, where it is sufficient to mask some portion of the input randomly and reconstruct the input. 
Earth observation data differs from these domains in having aligned yet highly multi-modal, multi-temporal data. 
A uniform masking strategy over all tokens may be too easy because a token will have many similar tokens either in space, time, or at a different aligned modality~\cite{tseng2025galileo}.
We adjust our masking strategy to limit the amount of context present in any sample without resorting to skewed masking ratios.


\noindent\textit{Contrasting against Earth tokens.}
Similarly, with our loss formulation we find a small adjustment makes a large difference in downstream performance. Similar to other SSL approaches operating in the latent space, we use a contrastive loss instead of a reconstruction loss. However, contrasting a reconstructed token against all other tokens in a batch, or even in the same sample, leads to many easy negatives given the highly redundant nature of multi-modal, multi-temporal Earth observation data. Instead, we contrast tokens only with other tokens corresponding to the same modality and bands. This focuses the model training on a more challenging but more productive objective.

\noindent\textbf{Comprehensive evaluation.}
There is no standard evaluation test suite for remote sensing models. While there are some established standard practices, they are not always followed. To get a more complete picture of the state of foundation model performance, we ran comprehensive evaluations across a variety of research benchmarks. Further, to evaluate real-world performance, we also evaluated models on datasets from $7$ partner organizations that use Earth observation modeling in their work.

Following standard practice, we evaluated all models using simple transfer learning techniques (kNN and linear probing) as well as full, end-to-end fine-tuning. We evaluated {\model} as well as other top-performing foundation models using a standard training recipe,  sweeping over a variety of parameter and settings to ensure a fair evaluation.

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.46\linewidth]{figures/knn_lp_summary.pdf}
    \includegraphics[width=0.5\linewidth]{figures/ft_summary.pdf}
    \caption{{\model} substantially outperforms previous remote sensing foundation models, both when using embeddings with kNN and linear probing, and with full fine-tuning. Here, we show the inverted rank averaged across tasks involving only Sentinel-2 images, which all models support.}
    \label{fig:result_summary}
\end{figure*}

Figure \ref{fig:result_summary} compares the models in terms of their inverted rank, averaged over all Sentinel-2 tasks (other tasks are only compatible with a subset of models). {\model} substantially outperforms all other remote sensing foundation models that we evaluated.

\noindent\textbf{Open platform.}
While multiple Earth observation models already exist, adoption is lagging behind, especially in the non-profit sector.
Some models are simply closed source and reproducing them would take an experienced research team and an expensive GPU cluster~\cite{brown2025alphaearth}. Even if the model code and weights are open, or embeddings are pre-computed and shared, applying a foundation model to a novel task requires data gathering, alignment, pre-processing, labeling, fine-tuning, and running inference. 

By contrast, all of the {\model} training code, model weights, training data, fine-tuning scripts, and even pre-trained weights are freely available.
Additionally, 
We built an end-to-end platform to simply this process for our partner organizations. The platform supports all the data wrangling needed to finetune and run inference on \model with customized data.
The {\platform} is an end-to-end solution for organizations who want to harness Earth observation data for the public good. 
Our partner organizations are already using the platform for things like mangrove conservation, ecosystem mapping, and food security prediction. This solves the last-mile problem of putting frontier research into the hands of people who can use it to do the most good.



==> sec/1_intro_3.tex <==
% THIS IS NOT THE INTRODUCTION YOU ARE LOOKING FOR...

\section{Introduction}
\label{sec:intro}

Earth observation foundation models show promising results in research settings \cite{astruc2024anysat, wang2025towards, fuller2024croma, tseng2025galileo, waldmann_shah_2025_panopticon, jakubik2025terramindlargescalegenerativemultimodality, feng2025tessera}.  However, adoption for real-world tasks lags behind, especially in the non-profit sector. Foundation models are large, complex to train, and expensive to deploy in computation and expertise.

To help enable non-profits to use these powerful tools we train {\model}, a new family of models, using a novel, stable training regime. We comprehensively evaluate {\model} against 12 other foundation models on both research benchmarks and real-world tasks from partner organizations. Finally we deploy these models in an open, end-to-end platform bringing frontier models directly to organizations who need it the most.

\subsection{Stable Training}

Foundation models are complex and expensive to train. When attempting to replicate existing work we frequently saw training instability, representation collapse, and models underperforming their stated potential. We introduce a stable training regime that models images in latent space to produce high-quality representations but avoids instability and collapse.

%Existing foundation model approaches either train in a supervised or unsupervised setting. Some foundation models are trained to predict supervised labels like land cover maps from satellite observations \cite{bastani2023satlaspretrain}. Other foundation models use the vast quantity of unlabeled data to train in a self-supervised manner \cite{wang2023ssl4eo}. We present a formulation that unifies these approaches into a single task, show that it works well with only observational data, and further improves when we add labels.

Our approach strikes a middle ground between two common approaches in self-supervised learning. Masked autoencoders (\textbf{MAE}) predict pixel-level reconstructions of masked input while approaches like \textbf{I-JEPA} and Latent Masked Image Modeling (\textbf{Latent MIM}) predict reconstructions in feature space \cite{assran2023self, wei2024towards}. MAE tends to be stable but limited in its feature representations while latent approaches are unstable but produce better features \cite{mo2024connecting}.

We present Latent Masked Image Modeling of Linear, Invariant Token Embeddings (\textbf{Latent MIM Lite}), a simplification of Latent MIM that leads to stable training and better performance. We replace the target encoder of Latent MIM with a linear projection from image patches to token space that is randomly initialized and never updated during training. This simple modification stabilizes training but maintains the representative power of modeling in latent space. It also unifies self-supervised and supervised learning as we project both observational data and labeled maps through the frozen random projection layer into token space and calculate loss the same for both.

\subsubsection{Masking}

Many foundation models build upon work in domains like image or text processing. Earth observation data differs from these domains in having spatially aligned yet highly multi-modal, multi-temporal data. We find that adjusting our masking strategy and loss to account for this unique domain gives us significantly better performance.

In image or text modeling it is sufficient to randomly mask some portion of the input and have the model reconstruct the input from context. With remote sensing data, any token in the input will have many similar tokens either in space, time, or at a different aligned modality. Random masking is too easy of a task unless you use a very high masking ratio \cite{tseng2025galileo}. We introduce a modality-aware masking strategy that combines random token masking with full modality reconstruction to make the task challenging without resorting to skewed masking ratios.

\subsubsection{Loss}

Like other SSL approaches in latent space we use a contrastive loss instead of a reconstruction loss. However, contrasting a reconstructed token against all other tokens in a batch, or even in the same sample, leads to many easy negatives given the redundant nature of Earth observation data. Instead we contrast tokens only with other tokens in their respective bandset (a subdivision of modality explained in \ref{subsec:data}). This focuses the model training on a more challenging but more productive objective as shown in our experiments.

\subsection{Comprehensive Evaluation}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.46\linewidth]{figures/knn_lp_summary.pdf}
    \includegraphics[width=0.5\linewidth]{figures/ft_summary.pdf}
    \caption{OlmoEarth substantially outperforms previous remote sensing foundation models, both when using embeddings (left), and with full fine-tuning (right). We show the inverted rank averaged across tasks involving Sentinel-2 images. We exclude tasks from the embedding evaluation that perform poorly without fine-tuning, such as object detection tasks. Due to compute constraints, we don't fine-tune large versions of models if a base model exists (including for {\model}).}
    \label{fig:result_summary}
\end{figure*}

There is no standard evaluation suite for remote sensing models. While there are some established standard practices \cite{reed2023scale,fuller2024croma,tseng2025galileo}, they are not always followed. To get a more complete picture of the state of foundation modeling we run a comprehensive evaluation effort of {\model} compared to 12 other foundation models on 18 research benchmarks. Further, to evaluate real-world performance we also evaluate models on 19 datasets from $7$ partner organizations that are using Earth observation modeling in their work.

Following standard practice we evaluate all models using simple transfer learning techniques (kNN and linear probing) as well as full, end-to-end fine-tuning. We evaluate all models using a standard training recipe and sweeping over a variety of hyperparameters, ensuring a fair evaluation. {\model} achieves the best performance in 15 of 24 tasks for the kNN/LP evaluation and 20 of 29 tasks for full fine-tuning. See Table \ref{fig:result_summary} for a summary.

\subsection{Open Platform}

Training and fine-tuning remain out of reach for most environmental and humanitarian non-profits. Applying a foundation model to a task requires data gathering, alignment, pre-processing, labeling, fine-tuning, and running inference. Usually this would require a GPU cluster, research team, and the resources to gather and label data. We deploy {\model} as part of the {\platform} to simplify and streamline this process.

The {\platform} is an end-to-end solution for organizations who want to harness Earth observation data for the public good. It encompasses all phases of Earth modeling, from data curation and labeling, to fine-tuning, inference, and deployment. Our partner organizations are already using the platform for things like mangrove conservation, ecosystem mapping, and agricultural planning for food security. The {\platform} solves the last-mile problem of putting frontier research into the hands of people who can use it to do the most good.


==> sec/1_intro_taylors_version.tex <==
\section{Introduction}
\label{sec:intro}

Everyone is training Earth observation foundation models these days \cite{astruc2024anysat, clayfoundation, wang2025towards, fuller2024croma, siméoni2025dinov3, tseng2025galileo, waldmann_shah_2025_panopticon, tseng2023lightweight, szwarcman2024prithvi, bastani2023satlaspretrain, jakubik2025terramindlargescalegenerativemultimodality, feng2025tessera, brown2025alphaearth} but they're all garbage. So we decided to train a better one. Our work offers three major contributions:

\begin{enumerate}
    \item Stable training in latent space with a novel target encoder, masking strategy, and loss.
    \item Large scale evaluation across a range of tasks and foundation models.
    \item Open model code, weights, training data, and an end-to-end platform to drive adoption.
\end{enumerate}

\subsection{Stable Training}

Existing foundation model approaches either train in a supervised or unsupervised setting. Some foundation models are trained to predict supervised labels like land cover maps from satellite observations \cite{bastani2023satlaspretrain}. Other foundation models use unlabeled observational data to train in a self-supervised manner \cite{wang2023ssl4eo}. We present a formulation that unifies these approaches into a single task, show that it works well with only observational data, and further improves when we add labels.

Our unified approach strikes a middle ground between two common approaches in self-supervised learning. Masked autoencoders (\textbf{MAE}) predict pixel-level reconstructions of masked input while approaches like \textbf{I-JEPA} and Latent Masked Image Modeling (\textbf{Latent MIM}) predict reconstructions in feature space \cite{assran2023self, wei2024towards}. MAE tends to be stable but limited in its feature representations, while latent approaches are unstable but produce better features (if they don't crash during training)~\cite{mo2024connecting}.

\subsubsection{Target Encoder}

We present Latent Masked Image Modeling of Linear, Invariant Token Embeddings (\textbf{Latent MIM Lite}), a simplification of Latent MIM that leads to stable training and better performance. We replace the target encoder of Latent MIM with a linear projection from image patches to token space that is randomly initialized and never updated during training. This simple modification stabilizes training but maintains the representative power of modeling in latent space. It also unifies self-supervised and supervised learning as we project both observational data and labeled maps through the frozen random projection layer into token space and calculate loss the same for both.

\subsubsection{Masking}

Many foundation models build upon work in domains like image or text processing. Earth observation data differs from these domains in having spatially aligned yet highly multi-modal, multi-temporal data. We find that adjusting our masking strategy and loss to account for this unique domain gives us significantly better performance.

In image or text modeling it is sufficient to randomly mask some portion of the input and have the model reconstruct the input from context. With remote sensing data, because we have aligned data over various modalities and timesteps, a uniform masking strategy over all tokens may be too easy of a task. Any token in the input will have many similar tokens either in space, time, or at a different aligned modality. There is too much context unless you use a very high masking ratio \cite{tseng2025galileo}. We adjust our masking strategy to limit the amount of context present in any sample by masking tokens within each modality. This makes the problem challenging without resorting to skewed masking ratios.

\subsubsection{Loss}

Similarly, with our loss formulation we find a small adjustment makes a large difference in downstream performance. Like other SSL approaches in latent space we use a contrastive loss instead of a reconstruction loss. However, contrasting a reconstructed token against all other tokens in a batch, or even in the same sample, leads to many easy negatives given the highly redundant nature of Earth observation data. Instead we contrast tokens only with other tokens in their respective bandset (a subdivision of modality explained in \autoref{subsec:data}). This focuses the model training on a more challenging but more productive objective.


\subsection{Comprehensive Evaluation}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/knn_lp_summary.pdf}
    \caption{{\model} substantially outperforms previous remote sensing foundation models. We show the average rank across tasks involving only Sentinel-2 images when using frozen embeddings (lower is better).}
    \label{fig:result_summary}
\end{figure}
% https://docs.google.com/spreadsheets/d/10n5DQ6f6ippwn3kKaD_ndebB2D7UHd_ZtW7ei_hogk4/edit?gid=303360532#gid=303360532 (see ranks across 13 tasks)

% Finetune figure: finetune_summary.pdf

There is no standard evaluation test suite for remote sensing models. While there are some established standard practices, they are not always followed. To get a more complete picture of the state of foundation modeling we run a comprehensive evaluation effort of {\model} compared to 12 other foundation models on 18 research benchmarks. Further, to evaluate real-world performance we also evaluate models on 19 datasets from $7$ partner organizations that are using Earth observation modeling in their work.

Following standard practice we evaluate all models using simple transfer learning techniques (kNN and linear probing) as well as full, end-to-end fine-tuning. We evaluate all models using a standard training recipe, and sweep over a variety of parameters, ensuring a fair evaluation.


We show detailed results in Section \ref{sec:experiments}.
{\model} achieves the best performance on 15 of 24 tasks for the kNN/LP evaluation and 20 of 29 tasks for full fine-tuning.
Figure \ref{fig:result_summary} summarizes the results in terms of average rank.

\subsection{Open Platform}

Again, everyone is training Earth observation models these days. But adoption is lagging behind, especially in the non-profit sector where organizations would love to use these models to solve big problems.

Some models are proprietary and reproducing them would take an experienced research team, a GPU cluster, and a lot of money \cite{brown2025alphaearth}. All of the {\model} pre-training code and data, fine-tuning scripts, and pre-trained weight files are freely available.

Even with model code and weights, applying a foundation model to a novel task requires data gathering, alignment, pre-processing, labeling, fine-tuning, and running inference. Do you know how to get data from a satellite? I sure don't. But someone on the team does and we built a whole end-to-end platform to get all that data and do all those other things too. Including running training and inference so our partners don't have to spin up a GPU cluster.

The {\platform} is an end-to-end solution for organizations who want to harness Earth observation data for the public good. Our partner organizations are already using the platform for things like mangrove conservation, ecosystem mapping, and agricultural planning for food security. This solves the last-mile problem of putting frontier research into the hands of people who can use it to do the most good.

\begin{comment}
Again, everyone is training earth observation models these days. But adoption is lagging behind, especially in the non-profit sector where organizations would love to use these models to solve big problems.

Some models are simply closed source and reproducing them would take an experienced research team, a GPU cluster, and a lot of money \cite{brown2025alphaearth}. All of the {\model} pre-training code and data, fine-tuning scripts, and pre-trained weight files are freely available.

Even with model code and weights, applying a foundation model to a novel task requires data gathering, alignment, pre-processing, labeling, fine-tuning, and running inference. Do you know how to get data from a satellite? I sure don't. But someone on the team does and we built a whole end-to-end platform to get all that data and do all those other things too. Including run training and inference so our partners don't have to buy thousands of dollars of GPU time.

The {\platform} is an end-to-end solution for organizations who want to harness earth observation data for the public good. Our partner organizations are already using the platform for things like mangrove conservation, ecosystem mapping, and food security prediction. This solves the last-mile problem of putting frontier research into the hands of people who can use it to do the most good.





Training foundation models is hard. Self-supervised learning (SSL) typically involves a tradeoff between stability of training and performance of the final model.

\subsubsection{MAE}

Masked autoencoders (MAE) learn to predict masked portions of the input in pixel-space with a reconstruction loss like Smooth-L1. This training formulation is often stable but limited in performance. 

Masked areas in pixel space have a wide range of possible values that are equally probable. Whether an edge exists an one location or another a few pixels away has little semantic difference but a large difference in the individual pixel values. Thus a lot of the loss is devoted to a task that is inherently very challenging but also of little semantic value. The reconstructions produced by such a model are often a blurry mess (due to minimizing L2 loss) while the features extracted by the model have limited semantic value.

\subsubsection{Latent MIM}

Latent Masked Image Modeling (Latent MIM) moves the reconstruction to latent space instead of pixel space. First an encoder converts the full, unmasked input into tokens or feature vectors. Then the model attempts to predict these tokens from a masked version of the input. Typically Latent MIM uses a contrastive loss instead of a reconstruction loss.

Reconstruction in latent space mitigates the issues with MAE. The model need not worry about precise details in pixel space and instead can focus on the semantically meaningful aspects of the task. For example, the existence of an edge and its approximate location and orientation will matter to the loss but not the precise pixels or their exact values.

However, Latent MIM faces a chicken and egg problem, to train an encoder for our foundation model (the \textbf{online encoder}) we need an encoder to produce the ground-truth features (the \textbf{target encoder}). In the standard formulation of Latent MIM the online encoder and target encoder share an overall architecture and the weights for the target encoder are an exponential moving average (EMA) of the online encoder. Loss is not propagated to the target encoder, it is only updated via EMA as the overall model trains.

This formulation is naturally unstable as there are obvious degenerate solutions. Updating the target encoder via EMA is meant to mitigate this but Latent MIM is still prone to collapse such that researchers have developed a variety of strategies to further address the issue.

\subsubsection{Latent MIM Lite}

We propose Latent Masked Image Modeling of Linear, Invariant Token Embeddings (Latent MIM Lite), a simplification of Latent MIM that leads to stable training and better performance. We replace the target encoder with a linear projection from image patches to token space that is randomly initialized and never updated during training.

Latent MIM Lite combines the stability of MAE training with the benefits of prediction in latent space. Randomly projecting raw input data extracts valuable features both from a theoretical and practical standpoint. Thus our predictions are operating in a true latent space of our input data. However, because we use a fixed target encoder we avoid the trivial solutions present in Latent MIM-style training. While it's possible this approach is too simplistic in more complex domains like natural image processing, empirical results show a clear benefit in our domain of earth observation data.

\subsection{Masking and Loss}

Masked image modeling requires masking the input, predicting something about the masked area, and calculating loss. Foundation models for image process spatial information, language models process sequential data (essentially time-series), and video models reason over space and time. Earth observation data is spatial, temporal, and additionally highly multi-modal. There are dozens of sources of open satellite data as well as derived products related to water, vegetation, land cover, and other maps.

The highly multi-modal nature of earth observation data 

\subsubsection{Modality-Aware Masking}

Most SSL foundation models are transformer-based so masking happens at token-level granularity, even for pixel-based reconstruction.


\end{comment}
\begin{comment}

Here's one overall way to frame the contributions:

\begin{itemize}
    \item motivation/applications first paragraph tbd
    \item broadly, existing foundation models fall into two classes, either employing a supervised learning strategy, where the model is trained to reproduce non-image raster data like land cover maps and street maps from satellite image inputs, or employing self-supervised learning. olmoearth combines self-supervised learning over satellite images with supervision from non-image rasters to boost performance.
    \item also, while existing foundation models are good, they haven't been adopted. one factor is the difficulty in obtaining satellite images that are processed in exactly the same way as the pre-training data. we release a library that contains code not only to fine-tune olmoearth, but also to ingest satellite images directly from data sources like the Copernicus and USGS EarthExplorer APIs, for target locations and time ranges of interest.
\end{itemize}


\begin{itemize}
    \item Henry/Joe: MAE is pretty good but reconstructing in latent space is better, it can be unstable though, so we have this middle ground where the fixed projection and supervised-ish modalities helps to stabilize the training.
    \item Henry: patch discrimination work well because it is like L2 loss for predicting representation but also adds additional signal to push the representations further apart.
    \item Joe: there may be two parts, the MAE one and also unifying all of the modalities (even though maps vs observations feel like they are disjointed), which has some interplay between them but could be two points. also make sure we can lead into talking a lot about our unique masking strategy.
    \item Joe: should say something to make sure people don't ask why we don't just do these in the natural image domain, e.g. train on ImageNet + SSL.
    \item Joe: have section that talks about a bunch of the things we tried that didn't work, kind of presenting story of how we arrived at this thing. Favyen: maybe that can go in appendix since otherwise it could break the story.
    \item Henry: think about what to name the training objective part of the approach.
\end{itemize}
\end{comment}


==> sec/anon.tex <==
\def\model{Helios}
\def\platform{Helios Platform}
\def\modelurl{\url{REDACTED}}
\toggletrue{anon}
\usepackage[review]{cvpr}      % To produce the REVIEW version

\def\colorone{aa1443}
\def\colortwo{1177aa}
\def\colorthree{0000ff}
\def\colorfour{00aa00}
\def\colorfive{aa7700}
\def\colorsix{44aa77}
\def\colordefault{000000}

\def\datamap{figures/datamap_anon.png}



==> sec/rank_vs_macs.tex <==
\definecolor{ourcolor}{HTML}{f0529c}
\definecolor{secondcolor}{HTML}{105257}
\definecolor{thirdcolor}{HTML}{b11bE8}

\begin{figure}[t]
    \vspace{-5pt}
    \centering
    \begin{tikzpicture}
        \begin{axis}[
            xmode=log,
            width=\columnwidth,
            height=7cm,
            xmin=0.223, xmax=1300, % Limits to cover the full date range
            ymin=2.5, ymax=16.25,
            xtick={1, 10, 100, 1000},
            % xticklabel style={anchor=north, /pgf/number format/precision=0, /pgf/number format/use comma=false, /pgf/number format/1000 sep={}}, % Ensures no commas and integer formatting
            xlabel={MACs ($
            \times 10^{9}$)},
            ylabel={Average Rank via $k$NN and LP},
            grid=major,
        ]
            % Scatter plot points with decimal year representation
            \addplot[only marks, mark=*, mark options={scale=1.2, color=secondcolor}] coordinates {(725.58, 14)}; % AnySat
            % Manually place labels at specified offsets
            \node[anchor=south, text=secondcolor] at (axis cs:725.6, 14) {\scriptsize AnySat};

            \addplot[only marks, mark=*, mark options={scale=1.2, color=secondcolor}] coordinates {(25.92, 15.77)}; % Clay
            \node[anchor=west, text=secondcolor] at (axis cs:25.9, 15.77) {\scriptsize Clay};

            \addplot[only marks, mark=*, mark options={scale=1.2, color=thirdcolor}] coordinates {(5.79, 10.23)}; % CopernicusFM
            \node[anchor=west, text=thirdcolor] at (axis cs:5.79, 10.23) {\scriptsize CopernicusFM};

            \addplot[only marks, mark=*, mark options={scale=1.2, color=secondcolor}] coordinates {(10.70, 6.61)}; % CROMA Base
            \node[anchor=east, text=secondcolor] at (axis cs:10.70, 6.61) {\scriptsize CROMA Base};

            \addplot[only marks, mark=*, mark options={scale=1.2, color=secondcolor}] coordinates {(38.08, 7.46)}; % CROMA Large
            \node[anchor=west, text=secondcolor] at (axis cs:38.08, 7.46) {\scriptsize CROMA Large};

            \addplot[only marks, mark=*, mark options={scale=1.2, color=secondcolor}] coordinates {(19.95, 12.85)}; % DINOv3 Sat Large
            \node[anchor=west, text=secondcolor] at (axis cs:19.95, 12.85) {\scriptsize DINOv3 Sat Large};

            \addplot[only marks, mark=*, mark options={scale=1.2, color=secondcolor}] coordinates {(412.44, 9.85)}; % DINOv3 Sat 7B
            \node[anchor=north, text=secondcolor] at (axis cs:300, 9.85) {\scriptsize DINOv3 Sat 7B};

            \addplot[only marks, mark=*, mark options={scale=1.2, color=secondcolor}] coordinates {(0.42, 12.54)}; % Galileo Nano
            \node[anchor=west, text=secondcolor] at (axis cs:0.42, 12.54) {\scriptsize Galileo Nano};

            \addplot[only marks, mark=*, mark options={scale=1.2, color=secondcolor}] coordinates {(2.86, 10)}; % Galileo Tiny
            \node[anchor=north, text=secondcolor] at (axis cs:2.86, 10) {\scriptsize Galileo Tiny};

            \addplot[only marks, mark=*, mark options={scale=1.2, color=thirdcolor}] coordinates {(45.61, 6.23)}; % Galileo Base
            \node[anchor=west, text=thirdcolor] at (axis cs:45.61, 6.23) {\scriptsize Galileo Base};

            \addplot[only marks, mark=*, mark options={scale=1.2, color=thirdcolor}] coordinates {(18.69, 6.77)}; % Panopticon
            \node[anchor=south, text=thirdcolor] at (axis cs:15, 6.77) {\scriptsize Panopticon};

            \addplot[only marks, mark=*, mark options={scale=1.2, color=secondcolor}] coordinates {(19.79, 13.69)}; % Prithvi v2
            \node[anchor=east, text=secondcolor] at (axis cs:19.79, 13.69) {\scriptsize Prithvi Large};

            \addplot[only marks, mark=*, mark options={scale=1.2, color=thirdcolor}] coordinates {(53.64, 13.46)}; % Prithvi v2
            \node[anchor=south, text=thirdcolor] at (axis cs:53.64, 13.46) {\scriptsize Prithvi Huge};

            \addplot[only marks, mark=*, mark options={scale=1.2, color=thirdcolor}] coordinates {(0.44, 15.69)}; % Satlas
            \node[anchor=south, text=thirdcolor] at (axis cs:0.44, 15.69) {\scriptsize Satlas};

            \addplot[only marks, mark=*, mark options={scale=1.2, color=secondcolor}] coordinates {(5.68, 7.23)}; % Terramind B
            \node[anchor=south, text=secondcolor] at (axis cs:5.68, 7.23) {\scriptsize TerraMind Base};

            \addplot[only marks, mark=*, mark options={scale=1.2, color=secondcolor}] coordinates {(19.85, 5.54)}; % Terramind L
            \node[anchor=north, text=secondcolor] at (axis cs:19.85, 5.54) {\scriptsize TerraMind Large};

            \addplot[only marks, mark=*, mark options={scale=1.2, color=ourcolor}] coordinates {(0.27, 7.92)}; % OlmoEarth Nano
            \node[anchor=south, text=ourcolor] at (axis cs:0.5, 7.92) {\scriptsize {\model} Nano};

            \addplot[only marks, mark=*, mark options={scale=1.2, color=ourcolor}] coordinates {(1.73, 7.23)}; % OlmoEarth Tiny
            \node[anchor=east, text=ourcolor] at (axis cs:1.73, 7.23) {\scriptsize {\model} Tiny};

            \addplot[only marks, mark=*, mark options={scale=1.2, color=ourcolor}] coordinates {(27.43, 2.69)}; % OlmoEarth Base
            \node[anchor=south, text=ourcolor] at (axis cs:27.43, 2.69) {\scriptsize {\model} Base};

            % draw the pareto front
            \draw[ourcolor,->] (0.27, 7.92) -- (1.73, 7.23) -- (27.43, 2.69);
        \end{axis}
    \end{tikzpicture}
    \vspace{-10pt}

    \caption{{\model} achieves a Pareto front on performance vs. computational efficiency. Performance is defined as average rank. Compute efficiency is average MACs requires to encode a single instance for each task. Colours are only to distinguish points. \ranjay{draw the pareto front.} {\color{blue} Gabi: how's this? (lines between points)}}
    % % Accuracy trades off with inference cost as patch size varies in $\{4, 8, 16\}$.
    % % % EuroSat accuracy by $k$NN trades off with inference cost as patch size varies in $\{4, 8, 16\}$.
    % % Cost is measured as Multiply-Accumulate operations (MACs) for encoding one EuroSat input (note the log scale on the x-axis).
    % % Galileo model size and patch size offer balance between performance and cost.
    % % See Table \ref{tab:eurosat_per_patch} for full results.
    % % % Practitioners can balance model performance with inference-time compute costs by varying the input patch size.
    % }
    \label{fig:result_summary}
\end{figure}

